Joint Embedding of Graphs

Feature extraction and dimension reduction for networks is critical in a wide variety of domains. Efficiently and accurately learning features for multiple graphs has important applications in statistical inference on graphs. We propose a method to jointly embed multiple undirected graphs. Given a set of graphs, the joint embedding method identifies a linear subspace spanned by rank one symmetric matrices and projects adjacency matrices of graphs into this subspace. The projection coefficients can be treated as features of the graphs, while the embedding components can represent vertex features. We also propose a random graph model for multiple graphs that generalizes other classical models for graphs. We show through theory and numerical experiments that under the model, the joint embedding method produces estimates of parameters with small errors. Via simulation experiments, we demonstrate that the joint embedding method produces features which lead to state of the art performance in classifying graphs. Applying the joint embedding method to human brain graphs, we find it extracts interpretable features with good prediction accuracy in different tasks.

==> Joint Embedding of Graphs - arxiv FINAL /latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );
 
        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );
 
        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
 
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
